Argumentation and Machine Learning

This chapter provides an overview of research works that present approaches with some degree of cross-fertilisation between Computational Argumentation and Machine Learning. Our review of the literature identified two broad themes representing the purpose of the interaction between these two areas: argumentation for machine learning and machine learning for argumentation. Across these two themes, we systematically evaluate the spectrum of works across various dimensions, including the type of learning and the form of argumentation framework used. Further, we identify three types of interaction between these two areas: synergistic approaches, where the Argumentation and Machine Learning components are tightly integrated; segmented approaches, where the two are interleaved such that the outputs of one are the inputs of the other; and approximated approaches, where one component shadows the other at a chosen level of detail. We draw conclusions about the suitability of certain forms of Argumentation for supporting certain types of Machine Learning, and vice versa, with clear patterns emerging from the review. Whilst the reviewed works provide inspiration for successfully combining the two fields of research, we also identify and discuss limitations and challenges that ought to be addressed in order to ensure that they remain a fruitful pairing as AI advances.

==> macros.tex <==
% Latex commands for abstract argumentation in HOFA - Draft proposal


% Some general notation

\newcommand{\card}[1]{\ensuremath{|#1|}}                      % cardinality of #1
\newcommand{\powset}[1]{\ensuremath{2^{#1}}}                  % powerset of #1
\newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}       % a tuple

% Argumentation framework structure and relations


\newcommand{\argfram}{AF}                          % symbol for a generic argumentation framework
\newcommand{\arguments}{\ensuremath{\mathit{Ar}}}                        % set of arguments of an argumentation framework
\newcommand{\setarg}{\arguments}                                % alias for the above

\newcommand{\attackrel}{\ensuremath{\mathit{att}}}                        %attack relation of  an argumentation framework
\newcommand{\attack}{\attackrel}                               % alias for the above

\newcommand{\attacks}[2]{#1 \attackrel #2}                  % denotes that #1 attacks #2
\newcommand{\argattacks}[3]{#1 \attackrel_{#3} #2}                % denotes that #1 attacks #2 in argumentation framework #3

\newcommand{\attackers}[1]{#1^{-}}  % The arguments attacking #1
\newcommand{\attacked}[1]{#1^{+}} % The arguments attacked by #1

\newcommand{\negattackrel}{\not\rightarrow}                 % negated attack relation
\newcommand{\negattacks}[2]{#1 \negattackrel #2}            % denotes that #1 does not attack #2

\newcommand{\restargfram}[2]{{#1}{\downarrow_{#2}}}          % restriction of  the arg. framework #1 to the set of arguments #2

\newcommand{\scc}[1]{\ensuremath{{\mathrm{SCCS}}_{#1}}} %the strongly connected components of the argumentation framework #1

% Argumentation semantics

\newcommand{\gensem}{{\mathcal{S}}} % A generic semantics

\newcommand{\genext}{{\mathcal{E}}} % A generic extension

\newcommand{\Lab}{\mathcal{L}\!\mathit{ab}} % a labelling function

\newcommand{\genlabset}{{\mathcal{L}}} % A generic set of labellings
\newcommand{\genlab}{\genlabset}  % alias for the above

\newcommand{\inn}{\mathtt{in}}		% the in label in labelling-based semantics
\newcommand{\out}{\mathtt{out}}		% the out label in labelling-based semantics
\newcommand{\undec}{\mathtt{undec}} % the und label in labelling-based semantics

\newcommand{\labelset}{\Lambda} % a set of labels
\newcommand{\setoflabellings}[2]{{\mathfrak{L}(#1,#2)}} % the set of all labellings using set of labels #1 for argumentation framework  #2


\newcommand{\setgenext}[2]{\genext_{#2}(#1)} % the set of extension of the argumentation framework #1 according to semantics #2

\newcommand{\setgenlab}[2]{\genlab_{#2}(#1)} % the set of labellings of the argumentation framework #1 according to  semantics #2

\newcommand{\argdefsem}[1]{\mathcal{DE}_{#1}} % the set of argumentation frameworks for which the semantics #1 prescribes a non-empty set of extensions

\newcommand{\argdefsemlab}[1]{\mathcal{DL}_{#1}} % the set of argumentation frameworks for which the semantics #1 prescribes a non-empty set of labellings


\newcommand{\setmaxi}[1]{\mathcal{MCF}(#1)}% maximal conflict-free sets of AF #1

\newcommand{\sadm}{\mathcal{AD}} %  symbol for admissible semantics
\newcommand{\snai}{\mathcal{NA}} %  symbol for naive semantics
\newcommand{\sst}{\mathcal{ST}} %  symbol for stable semantics
\newcommand{\scm}{\mathcal{CO}} %  symbol for complete semantics
\newcommand{\sgr}{\mathcal{GR}}  %  symbol for grounded semantics
\newcommand{\spr}{\mathcal{PR}}   %  symbol for preferred semantics
\newcommand{\sideal}{\mathcal{ID}}  %  symbol for ideal semantics
\newcommand{\ssemi}{\mathcal{SST}}  %  symbol for semi-stable semantics
\newcommand{\sstg}{\mathcal{STG}}  %  symbol for stage semantics
\newcommand{\sCFtwo}{\mathcal{CF}2} %  symbol for CF2 semantics
\newcommand{\sstgtwo}{\mathcal{STG}2} %  symbol for stage2 semantics


\newcommand{\carfun}[1]{\ensuremath{\mathrm{F}_{#1}}}                 % characteristic function of the arg. framework #1

\newcommand{\multicarfun}[2]{\ensuremath{\mathrm{F}^{#1}_{#2}}} % #1-th composition of the characteristic function of the arg. framework #2


% Arguments and sets of arguments

\newcommand{\Args}{\mathcal{A}\mathit{rgs}}    % a generic set of arguments - extensive indication

\newcommand{\arga}{a} % A generic argument
\newcommand{\argb}{b} % Another generic argument
\newcommand{\argc}{c} % and so on ...
\newcommand{\argd}{d} % ...
\newcommand{\arge}{e} % ...

\newcommand{\argseta}{S} % A generic set of arguments
\newcommand{\argsetb}{T} % Another generic set of arguments
\newcommand{\argsetc}{U} % and so on ...
\newcommand{\argsetd}{V} % ...
\newcommand{\argsete}{W} % ...

